Unsupervised data augmentation for object detection

Data augmentation has always been an effective way to overcome overfitting issue when the dataset is small. There are already lots of augmentation operations such as horizontal flip, random crop or even Mixup. However, unlike image classification task, we cannot simply perform these operations for object detection task because of the lack of labeled bounding boxes information for corresponding generated images. To address this challenge, we propose a framework making use of Generative Adversarial Networks(GAN) to perform unsupervised data augmentation. To be specific, based on the recently supreme performance of YOLOv4, we propose a two-step pipeline that enables us to generate an image where the object lies in a certain position. In this way, we can accomplish the goal that generating an image with bounding box label.

==> Unsupervised Data Augmentationfor Object Detection/exp.tex <==

\subsection{Experiment Setting}
    \paragraph{Dataset}
     We use VOC2007 as our dataset. It has totally 9k images where each image is labeled with several bounding boxes. We resize those images to $64\times64\times3$ before feeding into the discriminator. Given the coordinate of bounding box, we also generate mask of size $64\times64\times1$ to match the size of input images and then feed into the generator together. We will discuss the reason that we choose this setting in the Section 4.3.

    \paragraph{GAN Model}
    We adopt Unet generator and N-Layer discriminator from Pix2Pix. We also adopt gradient penalty as WGAN-GP because of its advantages in both performance and stability. Generator and discriminator are trained iteratively. The goal of training generator is to generate indistinguishable samples for discriminator while the goal of training discriminator is to make sure it recognize real samples correctly. 
    
    \paragraph{Detection Model}
    We adopt YOLOv4 as our detection model, which is both fast and accurate. As is observed from our experiments, the YOLOv4 model pretrained on COCO dataset is also suitable for detection on VOC2007 dataset since 20 classes of VOC2007 are actually a subset of the 80 classes of COCO. So during training, we made use of pretrained YOLOv4 model to help us calculate the object position loss.

\subsection{Results Analysis}

    \paragraph{Step one}
    Results of the first step are shown in Figure \ref{real_gen_compare}, where the left image is real and the right one is generated. As can be seen, our model can generate similar image as real image. Although human being can recognize the object in generated image, i.e., a horse, a rider and the prairie background, there are still many noise-like pixels inside the generated image. These pixels may largely affect the performance of detection model. This phenomenon might due to the usage of WGAN, where the unsuitable magnitude of gradient penalty may distract its weights. Then the generator may not be able to concentrate fully on the competitive game itself, but also need to fulfill the requirement of gradient penalty item.
    
    \begin{figure}[htbp]
        \centering
        \begin{minipage}[t]{0.48\textwidth}
            \centering
            \includegraphics[scale=2]{figs/ori64x64.png}
        \end{minipage}
        \begin{minipage}[t]{0.48\textwidth}
        \centering
            \includegraphics[scale=2]{figs/gen.png}
        \end{minipage}
    \caption{Outcome of 1st-step model. \textbf{Left:} Real image from VOC dataset after resizing into $64\times64\times3$. \textbf{Right:} Corresponding generated image from our model.}
    \label{real_gen_compare}
    \end{figure}
    
    \paragraph{Step two} The results of second step are shown in Figure \ref{box_sample}. As shown in images, there is a rectangle in each generated image. This is because in the input of generator, we concatenate a mask to the noise in channel dimension. Without telling what generator shall do with this mask, it just automatically recognizes it as a shape it needs to display and thus there is an obvious boundary around the rectangle in each image. It is an interesting phenomenon, but it is actually not what we desired. In the future, one of our key directions is finding a better way to help generator understand the purpose of these input coordinates.
    
    \begin{figure}
      \centering
      \includegraphics[scale=0.3]{figs/box_sample.png}
      \caption{Temporary outcome of 2nd-step model.}
      \label{box_sample} 
     \end{figure}
    
\subsection{Discussion}

    In this part, we will analyze our problems met during experiment. 

    Initially, we were planning to generate larger images with size $256\times256\times3$. However, because of the limit of both time and available GPUs, after half month's trial, we decided to decrease it to $64\times64\times3$.
    
    It's well-known that GAN training is unstable. To address this, we've tried several methods to help stabilize the GAN training besides gradient penalty after our failure at the very beginning: learning rate decay after certain epochs and spectral normalization. Besides this, the largest problem is definitely about finding the balance between generator and discriminator.
    
    During training, we found that the discriminator outperforms generator most of the time even if we use the architectures proved to have similar capacity between generator and discriminator. The loss of such situation is shown in Figure \ref{training_curve}-left, where the generator cannot fool the discriminator after certain epochs. To address this, we use multiple tricks from internet, including adding Gaussian noise onto the input of discriminator, training generator with more steps at each iteration or just directly increasing the number of parameters of generator. However, it seems that this might relieve the problem to some degree, but the balance is still too fragile to maintain in our application. Most of the time, they compete with each other well at first, but after maybe several hours, things suddenly go wrong and the model just falls into the above situation that needs to stop and restart training.
    
    On the contrary, if we train the generator more frequently than discriminator, for example with a ratio of 3:1, then the loss curve will look like Figure \ref{training_curve}-right. It seems like this figure shows a perfect competition process, but actually, the generated images are even worse than the previous situation. The reason is that in this situation, the ability of discriminator is too poor to identify real images. A possible solution to these two situations is increasing both the number of discriminator steps and generator steps per iteration.
    
    What's more, compared to other application that use GAN for data augmentation, it seems that their GAN training is not so difficult as ours. One possible reason is that object detection dataset has more complex and distinct background between different images, which might confuse the generator a lot.
    
    \begin{figure}[htbp]
        \centering
        \begin{minipage}[t]{0.48\textwidth}
            \centering
            \includegraphics[scale=0.5]{figs/dbetterg.png}
        \end{minipage}
        \begin{minipage}[t]{0.48\textwidth}
        \centering
            \includegraphics[scale=0.6]{figs/gdsimilar.png}
        \end{minipage}
    \caption{Loss curve during our training. \textbf{Red:} score for real samples from discriminator. \textbf{Green and Blue:} score for fake samples from discriminator.}
    \label{training_curve}
    \end{figure}

            
\subsection{Future Work}

    From our perspectives, this topic is interesting and creative. So we are going to continue on this after this module if possible.
    %To our best knowledge, this is the first time  using GAN in data augmentation for object detection. 
    
    Our future work can be further extended in the following aspects:
    \begin{itemize}
        \item Continue on finding a better way to tell generator  the purpose of giving it those coordinates.
        \item Train a detection model based on augmented dataset to see if there are performance improvement compared to the case when only using original dataset.
        \item Further extend this framework, so that it can handle situation with multiple input coordinates and generate multiple objects on the generated image at the same time.

    \end{itemize}


==> Unsupervised Data Augmentationfor Object Detection/intro.tex <==


Computer Vision is one of the most important areas in Artificial Intelligence. It contains several basic tasks: image classification \cite{2015arXiv151203385H}, object detection \cite{2013arXiv1311.2524G}, instance segmentation \cite{2017arXiv170306870H} and semantic segmentation \cite{2014arXiv1412.7062C}. Among them, object detection has attracted widespread attention from researchers all over the world. It solves two main problems in real world applications: "What is the object?" and "Where is the object?". Current methods are simulating human vision and cognition in specific application scenarios, such as pedestrian detection, face detection and text detection. In recent years, with the development of deep learning technology, significant breakthroughs have been made in object detection, and it has also been applied to more fields such as automatic driving, robot vision, and video surveillance.

%\subsection{Motivation}
Although object detection has developed rapidly and new algorithms have constantly refreshing the scores of major rankings, one of its shortcomings is its difficulty in obtaining labeled data compared to classification task because of the tedious bounding box annotations process. A straight forward solution to this is generating pseudo label from trained detection model with confidence directly. However, it seems useless or even harmful since it's possible that the trained model will make mistake even if it gives out high confidence value.

During the survey, we found that some methods start using Generative Adversarial Network (GAN) for data augmentation recently, which achieve better results than traditional methods. For example, DAGAN \cite{antoniou2018data} succeed in generating augmented images for human face as shown in Figure \ref{DAGAN}, where only the left top one is real image. And after training on those augmented images, their model perform much better compared to those methods only using the real images. Inspired by these methods, we raise an enlightening question about this.

\begin{itemize}[leftmargin=*]
    %\noindent
    \item What if we can design a framework about GAN to generate augmented image together with the bounding box labels? 
\end{itemize}

To answer the above question, we develop a framework aiming to perform data augmentation for object detection based on the success of YOLOv4 and GAN. To be specific, we propose a two-step framework. In first step, our goal is to train a GAN for normal data augmentation based on original dataset, i.e., be able to generate real images. In second step, our goal is further extended to generate images where object should lies in certain position. And we use YOLOv4 to localize the position of object in the generated images and thus instruct the training of generator. With this model, the only thing we need to do is providing a position to the generator, then we can get the generated images that meet the requirement. Further more, we can use this technique to generate some hard samples, such as images with small or bias object. With these hard samples, model may become more robust after training.

In summary, the contributions of this paper are three folds:
\begin{itemize}
    \item Propose a novel data augmentation framework to solve the essential problem of lacking labeled sample in object detection.
    \item Encode the position constraint into the generated images.
    \item Provide comprehensive analysis and discussion on our results and experiment process, which should be useful to other people who are also new to this area.

\end{itemize}

To our best knowledge, this is the first work that applying GAN to generate the whole images directly based on a pure condition for object detection task.

==> exp.tex <==

\subsection{Experiment Setting}
    \paragraph{Dataset}
     We use VOC2007 as our dataset. It has totally 9k images where each image is labeled with several bounding boxes. We resize those images to $64\times64\times3$ before feeding into the discriminator. Given the coordinate of bounding box, we also generate mask of size $64\times64\times1$ to match the size of input images and then feed into the generator together. We will discuss the reason that we choose this setting in the Section 4.3.

    \paragraph{GAN Model}
    We adopt Unet generator and N-Layer discriminator from Pix2Pix. We also adopt gradient penalty as WGAN-GP because of its advantages in both performance and stability. Generator and discriminator are trained iteratively. The goal of training generator is to generate indistinguishable samples for discriminator while the goal of training discriminator is to make sure it recognize real samples correctly. 
    
    \paragraph{Detection Model}
    We adopt YOLOv4 as our detection model, which is both fast and accurate. As is observed from our experiments, the YOLOv4 model pretrained on COCO dataset is also suitable for detection on VOC2007 dataset since 20 classes of VOC2007 are actually a subset of the 80 classes of COCO. So during training, we made use of pretrained YOLOv4 model to help us calculate the object position loss.

\subsection{Results Analysis}

    \paragraph{Step one}
    Results of the first step are shown in Figure \ref{real_gen_compare}, where the left image is real and the right one is generated. As can be seen, our model can generate similar image as real image. Although human being can recognize the object in generated image, i.e., a horse, a rider and the prairie background, there are still many noise-like pixels inside the generated image. These pixels may largely affect the performance of detection model. This phenomenon might due to the usage of WGAN, where the unsuitable magnitude of gradient penalty may distract its weights. Then the generator may not be able to concentrate fully on the competitive game itself, but also need to fulfill the requirement of gradient penalty item.
    
    \begin{figure}[htbp]
        \centering
        \begin{minipage}[t]{0.48\textwidth}
            \centering
            \includegraphics[scale=2]{figs/ori64x64.png}
        \end{minipage}
        \begin{minipage}[t]{0.48\textwidth}
        \centering
            \includegraphics[scale=2]{figs/gen.png}
        \end{minipage}
    \caption{Outcome of 1st-step model. \textbf{Left:} Real image from VOC dataset after resizing into $64\times64\times3$. \textbf{Right:} Corresponding generated image from our model.}
    \label{real_gen_compare}
    \end{figure}
    
    \paragraph{Step two} The results of second step are shown in Figure \ref{box_sample}. As shown in images, there is a rectangle in each generated image. This is because in the input of generator, we concatenate a mask to the noise in channel dimension. Without telling what generator shall do with this mask, it just automatically recognizes it as a shape it needs to display and thus there is an obvious boundary around the rectangle in each image. It is an interesting phenomenon, but it is actually not what we desired. In the future, one of our key directions is finding a better way to help generator understand the purpose of these input coordinates.
    
    \begin{figure}
      \centering
      \includegraphics[scale=0.3]{figs/box_sample.png}
      \caption{Temporary outcome of 2nd-step model.}
      \label{box_sample} 
     \end{figure}
    
\subsection{Discussion}

    In this part, we will analyze our problems met during experiment. 

    Initially, we were planning to generate larger images with size $256\times256\times3$. However, because of the limit of both time and available GPUs, after half month's trial, we decided to decrease it to $64\times64\times3$.
    
    It's well-known that GAN training is unstable. To address this, we've tried several methods to help stabilize the GAN training besides gradient penalty after our failure at the very beginning: learning rate decay after certain epochs and spectral normalization. Besides this, the largest problem is definitely about finding the balance between generator and discriminator.
    
    During training, we found that the discriminator outperforms generator most of the time even if we use the architectures proved to have similar capacity between generator and discriminator. The loss of such situation is shown in Figure \ref{training_curve}-left, where the generator cannot fool the discriminator after certain epochs. To address this, we use multiple tricks from internet, including adding Gaussian noise onto the input of discriminator, training generator with more steps at each iteration or just directly increasing the number of parameters of generator. However, it seems that this might relieve the problem to some degree, but the balance is still too fragile to maintain in our application. Most of the time, they compete with each other well at first, but after maybe several hours, things suddenly go wrong and the model just falls into the above situation that needs to stop and restart training.
    
    On the contrary, if we train the generator more frequently than discriminator, for example with a ratio of 3:1, then the loss curve will look like Figure \ref{training_curve}-right. It seems like this figure shows a perfect competition process, but actually, the generated images are even worse than the previous situation. The reason is that in this situation, the ability of discriminator is too poor to identify real images. A possible solution to these two situations is increasing both the number of discriminator steps and generator steps per iteration.
    
    What's more, compared to other application that use GAN for data augmentation, it seems that their GAN training is not so difficult as ours. One possible reason is that object detection dataset has more complex and distinct background between different images, which might confuse the generator a lot.
    
    \begin{figure}[htbp]
        \centering
        \begin{minipage}[t]{0.48\textwidth}
            \centering
            \includegraphics[scale=0.5]{figs/dbetterg.png}
        \end{minipage}
        \begin{minipage}[t]{0.48\textwidth}
        \centering
            \includegraphics[scale=0.6]{figs/gdsimilar.png}
        \end{minipage}
    \caption{Loss curve during our training. \textbf{Red:} score for real samples from discriminator. \textbf{Green and Blue:} score for fake samples from discriminator.}
    \label{training_curve}
    \end{figure}

            
\subsection{Future Work}

    From our perspectives, this topic is interesting and creative. So we are going to continue on this after this module if possible.
    %To our best knowledge, this is the first time  using GAN in data augmentation for object detection. 
    
    Our future work can be further extended in the following aspects:
    \begin{itemize}
        \item Continue on finding a better way to tell generator  the purpose of giving it those coordinates.
        \item Train a detection model based on augmented dataset to see if there are performance improvement compared to the case when only using original dataset.
        \item Further extend this framework, so that it can handle situation with multiple input coordinates and generate multiple objects on the generated image at the same time.

    \end{itemize}

